Mechanical principles of dynamic terrestrial self-righting using wings

Terrestrial animals and robots are susceptible to flipping-over during rapid locomotion in complex terrains. However, small robots are less capable of self-righting from an upside-down orientation compared to small animals like insects. Inspired by the winged discoid cockroach, we designed a new robot that opens its wings to self-right by pushing against the ground. We used this robot to systematically test how self-righting performance depends on wing opening magnitude, speed, and asymmetry, and modeled how kinematic and energetic requirements depend on wing shape and body/wing mass distribution. We discovered that the robot self-rights dynamically using kinetic energy to overcome potential energy barriers, that larger and faster symmetric wing opening increases self-righting performance, and that opening wings asymmetrically increases righting probability when wing opening is small. Our results suggested that the discoid cockroach's winged self-righting is a dynamic maneuver. While the thin, lightweight wings of the discoid cockroach and our robot are energetically sub-optimal for self-righting compared to tall, heavy ones, their ability to open wings saves them substantial energy compared to if they had static shells. Analogous to biological exaptations, our study provided a proof-of-concept for terrestrial robots to use existing morphology in novel ways to overcome new locomotor challenges.

==> 2017 AR/2017AR_v5.tex <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@rmstyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand\BIBentrySTDinterwordspacing{\spaceskip=0pt\relax}
\providecommand\BIBentryALTinterwordstretchfactor{4}
\providecommand\BIBentryALTinterwordspacing{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand\BIBforeignlanguage[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}

\bibitem{Li2016cockroach}
C.~Li, C.~C. Kessens, A.~Young, R.~S. Fearing, and R.~J. Full,
  ``{Cockroach-inspired robot reveals principles of ground-based, dynamic
  self-righting},'' \emph{IEEE/RSJ International Conference on Intelligent
  Robots and Systems}, pp. 2128--2134, 2016.

\bibitem{brooks2004robots}
\BIBentryALTinterwordspacing
R.~Brooks, ``{The robots are here},'' \emph{Technology Review}, 2004.
\BIBentrySTDinterwordspacing

\bibitem{Siciliano2016handbook}
B.~Siciliano and O.~Khatib, \emph{{Springer Handbook of Robotics}}, 2016.

\bibitem{Saranli2001rhex}
\BIBentryALTinterwordspacing
U.~Saranli, M.~Buehler, and D.~E. Koditschek, ``{RHex: A Simple and Highly
  Mobile Hexapod Robot},'' \emph{The International Journal of Robotics
  Research}, vol.~20, no.~7, pp. 616--631, 2001.
\BIBentrySTDinterwordspacing

\bibitem{murphy2010trial}
\BIBentryALTinterwordspacing
R.~R. MURPHY, ``{Trial by fire:},'' \emph{Acta crystallographica. Section F,
  Structural biology and crystallization communications}, vol.~66, no. Pt 5,
  pp. 615--20, 2010.
\BIBentrySTDinterwordspacing

\bibitem{Huang2011operation}
\BIBentryALTinterwordspacing
Y.-w. Huang, Y.~Sasaki, Y.~Harakawa, E.~F. Fukushima, and S.~Hirose,
  ``{Operation of Underwater Rescue Robot Anchor Diver III during the 2011
  Tohoku Earthquake and Tsunami},'' \emph{Oceans 2011}, pp. 1--6, 2011.
\BIBentrySTDinterwordspacing

\bibitem{Wood2013flight}
\BIBentryALTinterwordspacing
R.~Wood, R.~Nagpal, and G.-Y. Wei, ``{Flight of the Robobees},''
  \emph{Scientific American}, vol. 308, no.~3, pp. 60--65, 2013.
\BIBentrySTDinterwordspacing

\bibitem{Low2015Perspectives}
\BIBentryALTinterwordspacing
K.~H. Low, T.~Hu, S.~Mohammed, J.~Tangorra, and M.~Kovac, ``{Perspectives on
  biologically inspired hybrid and multi-modal locomotion},''
  \emph{Bioinspiration {\&} Biomimetics}, vol.~10, no.~2, p. 020301, 2015.
\BIBentrySTDinterwordspacing

\bibitem{Astrand2002agricultural}
B.~{\AA}strand and A.~J. Baerveldt, ``{An agricultural mobile robot with
  vision-based perception for mechanical weed control},'' \emph{Autonomous
  Robots}, vol.~13, no.~1, pp. 21--35, 2002.

\bibitem{Billingsley2008robotics}
J.~Billingsley, A.~Visala, and M.~Dunn, ``{Robotics in Agriculture and
  Forestry},'' \emph{Springer handbook of robotics}, pp. 1065--1077, 2008.

\bibitem{Emmi2013Fleets}
\BIBentryALTinterwordspacing
L.~Emmi, L.~Paredes-Madrid, A.~Ribeiro, G.~Pajares, and P.~Gonzalez-de Santos,
  ``{Fleets of robots for precision agriculture: a simulation environment},''
  \emph{Industrial Robot: An International Journal}, vol.~40, no.~1, pp.
  41--58, 2013.
\BIBentrySTDinterwordspacing

\bibitem{Lauder2007fish}
\BIBentryALTinterwordspacing
G.~V. Lauder, E.~J. Anderson, J.~Tangorra, and P.~G.~a. Madden, ``{Fish
  biorobotics: kinematics and hydrodynamics of self-propulsion.}''
  \emph{Journal of Experimental Biology}, vol. 210, no. Pt 16, pp. 2767--2780,
  aug 2007.
\BIBentrySTDinterwordspacing

\bibitem{Moored2011Batoid}
\BIBentryALTinterwordspacing
K.~W. Moored, F.~E. Fish, T.~H. Kemp, and H.~Bart-Smith, ``{Batoid Fishes:
  Inspiration for the Next Generation of Underwater Robots},'' \emph{Marine
  Technology Society Journal}, vol.~45, no.~4, pp. 99--109, jul 2011.
\BIBentrySTDinterwordspacing

\bibitem{Kim2008smooth}
S.~Kim, S.~Member, M.~Spenko, S.~Trujillo, B.~Heyneman, D.~Santos, and M.~R.
  Cutkosky, ``{Smooth Vertical Surface Climbing With Directional Adhesion},''
  vol.~24, no.~1, pp. 65--74, 2008.

\bibitem{Rollinson2014pipe}
D.~Rollinson and H.~Choset, ``{Pipe Network Locomotion with a Snake Robot},''
  vol.~00, no.~0, pp. 1--15, 2014.

\bibitem{Trevelyan1997robots}
\BIBentryALTinterwordspacing
J.~Trevelyan, ``{Robots and landmines},'' \emph{Industrial Robot}, vol.~24,
  no.~2, pp. 114----{\&}, 1997.
\BIBentrySTDinterwordspacing

\bibitem{Zeng2007research}
J.~J. Zeng, R.~Q. Yang, W.~J. Zhang, X.~H. Weng, and Q.~Jun, ``{Research on
  semi-automatic bomb fetching for an EOD robot},'' \emph{International Journal
  of Advanced Robotic Systems}, vol.~4, no.~2, pp. 247--252, 2007.

\bibitem{matson2010unfree}
J.~Matson, ``{Unfree Spirit: NASA's Mars Rover Appears Stuck for Good},''
  \emph{Scientific American}, vol. 302, no.~4, pp. 16--18, 2010.

\bibitem{Bostock2014month}
M.~Bostock, S.~Carter, J.~Corum, and J.~White, ``{28 Months on Mars},''
  \emph{The New York Times}, 2014.

\bibitem{li2009sensitive}
C.~Li, P.~B. Umbanhowar, H.~Komsuoglu, D.~E. Koditschek, and D.~I. Goldman,
  ``{Sensitive dependence of the motion of a legged robot on granular media},''
  \emph{Proceedings of the National Academy of Sciences}, vol. 106, no.~9, pp.
  3029--3034, 2009.

\bibitem{Roberts2014deserta}
S.~Roberts, J.~Duperret, X.~Li, H.~Wang, and D.~Koditschek, ``{Desert RHex
  Technical Report : Tengger Desert Trip List of Figures},'' pp. 1--15, 2014.

\bibitem{Yang2011experimental}
R.~Yang, M.~Xu, X.~Liang, S.~Zhang, Y.~Cheng, H.~Xu, and J.~Yang,
  ``{Experimental study and DEM analysis on rigid driving wheel's performance
  for off-road vehicles moving on loose soil},'' \emph{2011 IEEE International
  Conference on Mechatronics and Automation, ICMA 2011}, pp. 142--147, 2011.

\bibitem{McKenna2008Toroidal}
J.~C. McKenna, D.~J. Anhalt, F.~M. Bronson, H.~B. Brown, M.~Schwerin,
  E.~Shammas, and H.~Choset, ``{Toroidal skin drive for snake robot
  locomotion},'' \emph{Proceedings - IEEE International Conference on Robotics
  and Automation}, pp. 1150--1155, 2008.

\bibitem{Li2015terradynamically}
\BIBentryALTinterwordspacing
C.~Li, A.~O. Pullin, D.~W. Haldane, H.~K. Lam, R.~S. Fearing, and R.~J. Full,
  ``{Terradynamically streamlined shapes in animals and robots enhance
  traversability through densely cluttered terrain},'' \emph{Bioinspiration
  {\&} Biomimetics}, vol.~10, no.~4, p. 046003, 2015.
\BIBentrySTDinterwordspacing

\bibitem{Kim2007Walking}
J.~Y. Kim, I.~W. Park, and J.~H. Oh, ``{Walking control algorithm of biped
  humanoid robot on uneven and inclined floor},'' \emph{Journal of Intelligent
  and Robotic Systems: Theory and Applications}, vol.~48, no.~4, pp. 457--484,
  2007.

\bibitem{Raibert2008BigDog}
\BIBentryALTinterwordspacing
M.~Raibert, K.~Blankespoor, G.~Nelson, R.~Playter, and t.~B. Team, ``{Bigdog,
  the rough-terrain quadruped robot},'' \emph{Proceedings of the 17th
  International Federation of Automation Control}, pp. 10\,822--10\,825, 2008.
\BIBentrySTDinterwordspacing

\bibitem{Bares1999dante}
J.~E. Bares and D.~Wettergreen, ``{Dante II : Technical Description, Results,
  and Lessons Learned},'' \emph{The International Journal of Robotics
  Research}, vol.~18, no.~7, pp. 621--649, 1999.

\bibitem{Chew1999Blind}
C.-M. C. C.-M. Chew, J.~Pratt, and G.~Pratt, ``{Blind walking of a planar
  bipedal robot on sloped terrain},'' \emph{Proceedings 1999 IEEE International
  Conference on Robotics and Automation (Cat. No.99CH36288C)}, vol.~1, no. May,
  pp. 1--6, 1999.

\bibitem{Peters2008Mobile}
S.~C. Peters and K.~Iagnemma, ``{Mobile robot path tracking of aggressive
  maneuvers on sloped terrain},'' \emph{2008 IEEE/RSJ International Conference
  on Intelligent Robots and Systems, IROS}, pp. 242--247, 2008.

\bibitem{spagna2007distributed}
\BIBentryALTinterwordspacing
J.~C. Spagna, D.~I. Goldman, P.-C. Lin, D.~E. Koditschek, and R.~J. Full,
  ``{Distributed mechanical feedback in arthropods and robots simplifies
  control of rapid running on challenging terrain.}'' \emph{Bioinspiration {\&}
  Biomimetics}, vol.~2, no.~1, pp. 9--18, 2007.
\BIBentrySTDinterwordspacing

\bibitem{Pettersen2011snake}
K.~Y. Pettersen, S.~Member, and {\O}.~Stavdahl, ``{Snake Robot Locomotion in
  Environments with Obstacles},'' \emph{IEEE TRANSACTIONS ON MECHATRONICS},
  vol.~XX, pp. 1--12, 2011.

\bibitem{Travers2016Shape}
M.~Travers, J.~Whitman, P.~Schiebel, D.~Goldman, and H.~Choset, ``{Shape-Based
  Compliance in Locomotion},'' \emph{Robotics: Science and Systems}, 2016.

\bibitem{li2013terradynamics}
C.~Li, T.~Zhang, and D.~I. Goldman, ``{A Terradynamics of Legged Locomotion on
  Granular Media},'' \emph{Science}, vol. 339, no. 6126, pp. 1408--1412, 2013.

\bibitem{Gong2015Simplifying}
\BIBentryALTinterwordspacing
C.~Gong, D.~I. Goldman, and H.~Choset, ``{Simplifying Gait Design via Shape
  Basis Optimization},'' \emph{Robotics: Science {\&} Systems}, vol.~15,
  no.~11, pp. 27\,738--27\,759, 2015.
\BIBentrySTDinterwordspacing

\bibitem{Bermudez2012Performance}
\BIBentryALTinterwordspacing
F.~Bermudez, R.~C.~R. Julian, D.~W.~D. Haldane, F.~L. {Garcia Bermudez},
  P.~Abbeel, and R.~S. Fearing, ``{Performance analysis and terrain
  classification for a legged robot over rough terrain},'' \emph{2012 IEEE/RSJ
  International Conference on Intelligent Robots and Systems}, pp. 513--519,
  oct 2012.
\BIBentrySTDinterwordspacing

\bibitem{Guizzo2015hard}
E.~Guizzo and E.~Ackerman, ``{The Hard Lessons of DARPA ' s Robotics
  Challenge},'' \emph{IEEE Spectrum}, vol.~52, no.~8, pp. 11--13, 2015.

\bibitem{Brown1998bow}
B.~Brown and G.~Zeglin, ``{The bow leg hopping robot},'' \emph{Proceedings.
  1998 IEEE International Conference on Robotics and Automation (Cat.
  No.98CH36146)}, vol.~1, no. May, 1998.

\bibitem{Fiorini2003development}
P.~Fiorini and J.~Burdick, ``{The development of hopping capabilities for small
  robots},'' \emph{Autonomous Robots}, vol.~2, no.~14, pp. 239--254, 2003.

\bibitem{Aoyama2005Micro}
H.~Aoyama, A.~Himoto, R.~Misumi, O.~Fuchiwaki, D.~Misaki, and T.~Sumrall,
  ``{Micro hopping robot with ir sensor for disaster survivor detection},''
  \emph{Proceedings of the 2005 IEEE International Workshop on Safety, Security
  and Rescue Robotics}, vol. 2005, no. June, pp. 189--194, 2005.

\bibitem{wallace2007Biologically}
M.~I. Wallace, J.~F. Burn, R.~A. Hyde, C.~Melhuish, and T.~Pipe,
  ``{Biologically Inspired Solutions for Compliant Limb UGVs},'' 2007.

\bibitem{Kovac2009steerable}
\BIBentryALTinterwordspacing
M.~Kovac, M.~Schlegel, J.-C. Zufferey, and D.~Floreano, ``{Steerable miniature
  jumping robot},'' \emph{Autonomous Robots}, vol.~28, no.~3, pp. 295--306, dec
  2009.
\BIBentrySTDinterwordspacing

\bibitem{Beyer2009performance}
E.~Beyer and M.~Costello, ``{Performance of a Hopping Rotochute},''
  \emph{International Journal of Micro Air Vehicles}, vol.~1, no.~2, pp.
  121--137, 2009.

\bibitem{Kessens2013Framework}
C.~C. Kessens, D.~C. Smith, and P.~R. Osteen, ``{A Framework for Autonomous
  Self-Righting of a Generic Robot on Sloped Planar Surfaces},'' \emph{IEEE
  International Conference on Robotics and Automation}, pp. 4724--4729, 2012.

\bibitem{Kossett2011robust}
A.~Kossett and N.~Papanikolopoulos, ``{A robust miniature robot design for
  land/air hybrid locomotion},'' \emph{IEEE International Conference on
  Robotics and Automation}, pp. 4595--4600, 2011.

\bibitem{Klaptocz2012Active}
\BIBentryALTinterwordspacing
A.~Klaptocz, L.~Daler, A.~Briod, J.-c. Zufferey, and D.~Floreano, ``{An Active
  Uprighting Mechanism for Flying Robots},'' \emph{IEEE Transactions on
  Robotics}, vol.~28, no.~5, pp. 1152--1157, 2012.
\BIBentrySTDinterwordspacing

\bibitem{Zhang2012self}
J.~Zhang, G.~Song, Z.~Li, G.~Qiao, H.~Sun, and A.~Song, ``{Self-righting,
  steering and takeoff angle adjusting for a jumping robot},'' \emph{IEEE
  International Conference on Intelligent Robots and Systems}, pp. 2089--2094,
  2012.

\bibitem{Briod2012AirBurr}
A.~Briod, A.~Klaptocz, J.~C. Zufferey, and D.~Floreano, ``{The AirBurr: A
  flying robot that can exploit collisions},'' \emph{2012 ICME International
  Conference on Complex Medical Engineering, CME 2012 Proceedings}, pp.
  569--574, 2012.

\bibitem{Krummel2014horseshoe}
G.~Krummel, K.~N. Kaipa, and S.~K. Gupta, ``{A Horseshoe Crab Inspired Surf
  Zone Robot with Righting Capabilities},'' in \emph{ASME International Design
  Engineering Technical Conferences and Computers and Information in
  Engineering Conference}, 2014, p. V05AT08A010.

\bibitem{peng2015motion}
\BIBentryALTinterwordspacing
S.~Peng, X.~Ding, F.~Yang, and K.~Xu, ``{Motion planning and implementation for
  the self-recovery of an overturned multi-legged robot},'' \emph{Robotica},
  vol.~5, pp. 1--14, 2015.
\BIBentrySTDinterwordspacing

\bibitem{Tunstel1999evolution}
\BIBentryALTinterwordspacing
E.~Tunstel, ``{Evolution of autonomous self-righting behaviors for articulated
  nanorovers},'' \emph{Proc. Fifth International Symposium on Artificial
  Intelligence.}, vol. 440, pp. 341--346, 1999.
\BIBentrySTDinterwordspacing

\bibitem{Schempf1999pandora}
H.~Schempf, E.~Mutschler, C.~Piepgras, J.~Warwick, B.~Chemel, S.~Boehmke,
  W.~Crowley, R.~Fuchs, and J.~Guyot, ``{Pandora: autonomous urban robotic
  reconnaissance system},'' \emph{IEEE International Conference on Robotics and
  Automation}, vol.~3, pp. 2315--2321, 1999.

\bibitem{Zong2006Realization}
G.~Zong, Z.~Deng, and W.~Wang, ``{Realization of a modular reconfigurable robot
  for rough terrain},'' \emph{IEEE International Conference on Mechatronics and
  Automation}, vol. 2006, pp. 289--294, 2006.

\bibitem{Yim2007towards}
M.~Yim, B.~Shirmohammadi, J.~Sastra, M.~Park, M.~Dugan, and C.~J. Taylor,
  ``{Towards robotic self-reassembly after explosion},'' \emph{IEEE/RSJ
  International Conference on Intelligent Robots and Systems}, pp. 2767--2772,
  2007.

\bibitem{Saranli2004model}
\BIBentryALTinterwordspacing
U.~Saranli, A.~Rizzi, and D.~E. Koditschek, ``{Model-Based Dynamic
  Self-Righting Maneuvers for a Hexapedal Robot},'' \emph{The International
  Journal of Robotics Research}, vol.~23, no.~9, pp. 903--918, 2004.
\BIBentrySTDinterwordspacing

\bibitem{Ben-Tzvi2008Design}
P.~Ben-Tzvi, A.~a. Goldenberg, and J.~W. Zu, ``{Design, simulations and
  optimization of a tracked mobile robot manipulator with hybrid locomotion and
  manipulation capabilities},'' \emph{IEEE International Conference on Robotics
  and Automation}, pp. 2307--2312, 2008.

\bibitem{Tsukagoshi2005Design}
H.~Tsukagoshi, M.~Sasaki, A.~Kitagawa, and T.~Tanaka, ``{Design of a higher
  jumping rescue robot with the optimized pneumatic drive},'' in \emph{IEEE
  International Conference on Robotics and Automation}, 2005, pp. 1276--1283.

\bibitem{kim2006isprawl}
\BIBentryALTinterwordspacing
S.~Kim, J.~E. Clark, and M.~R. Cutkosky, ``{iSprawl: Design and tuning for
  high-speed autonomous open-loop running},'' \emph{The International Journal
  of Robotics Research}, vol.~25, no.~9, pp. 903--912, 2006.
\BIBentrySTDinterwordspacing

\bibitem{Haldane2013Animal}
D.~W. Haldane, K.~C. Peterson, F.~L.~G. Bermudez, and R.~S. Fearing,
  ``{Animal-inspired Design and Aerodynamic Stabilization of a Hexapedal
  Millirobot},'' \emph{IEEE International Conference on Robotics and
  Automation}, pp. 3279--3286, 2013.

\bibitem{Kaspari1999size}
\BIBentryALTinterwordspacing
M.~Kaspari and M.~Weiser, ``{The size-grain hypothesis and interspecific
  scaling in ants},'' \emph{Functional Ecology}, vol.~13, no.~4, pp. 530--538,
  1999.
\BIBentrySTDinterwordspacing

\bibitem{blickhan1989spring}
R.~Blickhan, ``{The spring-mass model for running and hopping},'' \emph{Journal
  of Biomechanics}, vol.~22, no. 11-12, pp. 1217--1227, 1989.

\bibitem{Saranli2004multipoint}
\BIBentryALTinterwordspacing
U.~Saranli, A.~A. Rizzi, and D.~E. Koditschek, ``{Multi-point contact models
  for dynamic self-righting of a Hexapod},'' \emph{Springer Tracts in Advanced
  Robotics}, vol.~17, pp. 409--424, 2004.
\BIBentrySTDinterwordspacing

\bibitem{Johnson2013legged}
A.~M. Johnson and D.~E. Koditschek, ``{Legged Self-Manipulation},'' in
  \emph{IEEE Access}, vol.~1, no.~33, 2013, pp. 310--334.

\bibitem{li2015fast}
C.~Li, T.~Wohrl, H.~K. Lam, and R.~J. Full, ``{Fast, flipping cockroaches:
  dynamic, self-righting behavior},'' in \emph{Integrative and Comparative
  Biology}, vol.~55, 2015, p. E111.

\bibitem{Jay1982exaptation}
S.~Jay, E.~S. Vrba, S.~Paleobiology, N.~Winter, S.~J. Gould, and E.~S. Vrba,
  ``{Exaptation-A Missing Term in the Science of Form},'' \emph{Palaeontology},
  vol.~8, no.~1, pp. 4--15, 1982.

\bibitem{Brackenbury1990novel}
\BIBentryALTinterwordspacing
J.~Brackenbury, ``{A novel method of self-righting in the springtail Sminthurus
  viridis (Insecta: Collembola)},'' \emph{Journal of Zoology}, vol. 222, pp.
  117--119, 1990.
\BIBentrySTDinterwordspacing

\bibitem{full1995maximum}
\BIBentryALTinterwordspacing
R.~Full, A.~Yamauchi, and D.~Jindrich, ``{Maximum single leg force production:
  cockroaches righting on photoelastic gelatin},'' \emph{The Journal of
  experimental biology}, vol. 198, no.~12, pp. 2441--2452, 1995.
\BIBentrySTDinterwordspacing

\bibitem{Frantsevich2004righting}
\BIBentryALTinterwordspacing
L.~Frantsevich, ``{Righting kinematics in beetles (Insecta: Coleoptera).}''
  \emph{Arthropod structure {\&} development}, vol.~33, no.~3, pp. 221--35,
  2004.
\BIBentrySTDinterwordspacing

\bibitem{Young2006effects}
\BIBentryALTinterwordspacing
J.~S. Young, L.~S. Peck, and T.~Matheson, ``{The effects of temperature on
  walking and righting in temperate and Antarctic crustaceans},'' \emph{Polar
  Biology}, vol.~29, no.~11, pp. 978--987, 2006.
\BIBentrySTDinterwordspacing

\bibitem{Domokos2008Geometry}
\BIBentryALTinterwordspacing
G.~Domokos and P.~L. V{\'{a}}rkonyi, ``{Geometry and self-righting of
  turtles.}'' \emph{Proceedings of The Royal Society of London B: Biological
  Sciences}, vol. 275, no. 1630, pp. 11--7, 2008.
\BIBentrySTDinterwordspacing

\bibitem{Kessens2014metric}
\BIBentryALTinterwordspacing
C.~C. Kessens, C.~T. Lennon, and J.~Collins, ``{A metric for self-rightability
  and understanding its relationship to simple morphologies},'' \emph{IEEE/RSJ
  International Conference on Intelligent Robots and Systems}, pp. 3699--3704,
  2014.
\BIBentrySTDinterwordspacing

\bibitem{Dickinson2000animals}
\BIBentryALTinterwordspacing
M.~H. Dickinson, C.~T. Farley, R.~J. Full, M.~A.~R. Koehl, R.~Kram, and
  S.~Lehman, ``{How animals move: An integrative view},'' \emph{Science}, vol.
  288, no. 5463, pp. 100--106, 2000.
\BIBentrySTDinterwordspacing

\bibitem{Mintchev2016adaptive}
S.~Mintchev and D.~Floreano, ``{Adaptive Morphology},'' no. September, 2016.

\bibitem{Aguilar2016review}
\BIBentryALTinterwordspacing
J.~Aguilar, T.~Zhang, F.~Qian, M.~Kingsbury, B.~McInroe, N.~Mazouchova, C.~Li,
  R.~Maladen, C.~Gong, M.~Travers, R.~L. Hatton, H.~Choset, P.~B. Umbanhowar,
  and D.~I. Goldman, ``{A review on locomotion robophysics: the study of
  movement at the intersection of robotics, soft matter and dynamical
  systems},'' \emph{Reports on Progress in Physics}, vol. 110001, pp. 1--61,
  2016.
\BIBentrySTDinterwordspacing

\bibitem{Sasaki2016Reciprocity}
\BIBentryALTinterwordspacing
M.~Sasaki and T.~Nonaka, ``{The Reciprocity of Environment and Action in
  Self-Righting Beetles: The Textures of the Ground and an Object, and the
  Claws},'' \emph{Ecological Psychology}, vol.~28, no.~2, pp. 78--107, 2016.
\BIBentrySTDinterwordspacing

\bibitem{Walthall1981receptors}
W.~W. Walthall and H.~B. Hartman, ``{Receptors and giant interneurons signaling
  gravity orientation information in the cockroach Arenivaga},'' \emph{Journal
  of Comparative Physiology A}, vol. 142, no.~3, pp. 359--369, 1981.

\vspace{1in}
\noindent
\href{https://youtu.be/aD4B9LHXQws}{Talk - https://youtu.be/aD4B9LHXQws}
  
\noindent
\href{https://youtu.be/_ph705NvEHg}{Video 1 - \text{https://youtu.be/\_ph705NvEHg}}
  
\noindent
\href{https://youtu.be/w9sObMHqXpc}{Video 2 - \text{https://youtu.be/w9sObMHqXpc}}
  

\end{thebibliography}


==> 2017 AR/Templates/CHANGES <==
Changelog for version 1.9
- changes for compatibility with the latest MLA edition; use "style=mla-new" to change the Works Cited to the new style
- added support for some common biblatex-chicago citation commands (\headlesscite, \textcite, etc.)
- added preliminary support for new entry types (@artwork, @audio, @image, @letter, @music)
- added style intelligence with source mapping:
    * the word "University" in publisher names will automatically shorten to "U"
    * the word "Press" in publisher names will automatically shorten to "P"
    * the phrase "University Press" in publisher names will automatically shorten to "UP"
    * certain words in publisher names--including "Company," "Corporation," "Incorporated", "Limited," and their 
      respective abbreviations--will not be printed
    * if an entry includes a URL pointing to a number of eprint domains--including include JSTOR, Project Muse, Adelaide 
      Online Books, Google Books, EBSCO Academic Search Complete, EBSCO LexisNexis, and the EBSCO MLA Database--
      biblatex-mla will correctly reformat it as an eprint
    * if an entry includes a URL pointing to a doi server, biblatex-mla will correctly reformat it as an doi reference

Changelog for version 1.6
- changes for compatibility with Biblatex 3.3+
- changed behavior of "mancitepar", which now defaults to false
- fixed buggy repetition of series field (hopefully)
- an upcoming version will provide support for more entrytypes and reflect changes made 
  in the 2016 MLA handbook

Changelog for version 1.5:
- changes for compatibility with Biblatex 2.5
- added entrytypes @online, @inbook, @bookinbook
- updated entrytypes @video, @review
- added epprinttype "jstor"
- added package options "noremoteinfo" and "mancitepar" 
- added hyperref linking to "Web" bibstring
- quashed lingering spacing errors, improved bibnamedash, and improved handling of starred
  autocites
- improved documentation, examples

Changelog for version 0.9.5:
- changes for compatibility with Biblatex 1.0
- further support for latest MLA edition (now default); use "showmedium=false" 
  package option to revert
- added Italian localization (from Andrea Marchitelli)
- new entry option "nodate" to trigger display of MLA-style "n.d."
- added support and MLA formatting for eprint sources from Project Muse (using
  "muse" as eprinttype); in the eprint field, include the full URL to the
  article
- preliminary conversion of documentation to Philipp Lehman's ltxdockit, as 
  previous documentation files were lost

Changelog for version 0.9:
- many changes for compatibility with Biblatex v.0.9
- introduced support for style from latest MLA edition (this was a major 
  undertaking)
- new "print", "web", and "generaleditor" bibstrings
- formatting for eprint sources from JSTOR and Google Books, as already 
  included in Biblatex
- support and formatting for eprint sources from eBooks@Adelaide (using 
  "adelaide" as eprinttype); in the eprint field, include the full URL to the
  article
- new package options "showmedium" and "guessmedium" for updated MLA support
- improved support for reprints
- improved support for multivolume entries, including change from using 
  origyear field to using eventdate field, and added support for general 
  editor as "generaleditor" editortype
- converted proceedings to use eventdate field

Changelog for version 0.8.1:
- did nothing but make 0.8 beta final to upgrade CTAN

Changelog for version 0.8 beta:
- added further examples from the MLA Handbook (6th edition). Almost all of
  the non-periodical examples in section 5.6.x (and many of the periodical
  examples in 5.7.x) contained therein can now be successfully re-created
  using biblatex-mla.
- nameaddon and authortype behavior standardized across entrytypes
- added bookauthor support for suppcollection and suppbook
- significantly improved handling of multivolume works
- further improved handling of "et al." There should now be a comma before 
  "et al." only in reversed (last-first) naming schemes. Standard (first-last)
  schemes and last-name only schemes will omit the comma.
- improved support for maintitle
- improved presentation of title in conference proceeding, where title ends in
  an abbreviation dot
- added preliminary support for "generaleditor" editortype in the language
  (lbx) files
- added preliminary support for "volstodate" string in the language (lbx)
  files, theoretically to be used when indicating total volume numbers of
  multi-volume works with open-ranged years
- added title format for reference books
- removed extra leading space before nameaddon brackets
- added support for formatting of open-ranged years (as suggested by 
  Philipp Lehman)
- added support for limiting remote info, using methods similar to
  biblatex-apa
- added totalnames support for translator field
- re-added hyperref support mistakenly disabled in version 0.7
- fixed many citereset problems (while potentially introducing others...)
- many citation macros tidied and future-proofed
- footnote presentation considerably more stable

Changelog for version 0.7 final:
- added examples from the MLA Handbook (6th edition)
- added support for origlocation, origpublisher, origtitle, and origlanguage
  to allow for reprints and translations. Biblatex-mla only uses the
  origlanguage field to trigger the use of \bibstring{transof} in place of
  \bibstring{reprintof} for reprinted articles and will not actually print the
  contents of the origlanguage field.
- re-added support for translators in articles (mistakenly lost in 0.6)
- added localization and bibstrings for "bytypecompilerandeditor" and
  "transof" (in addition to "typecompilerandeditor")
- significantly improved footnote support, bringing it inline with support for
  entries in the bibliography. This work is currently in progress, but non-
  periodical entries should be fully supported.
- in addition to Spanish and Portuguese localizations (contributed by Ivan
  Fernandez and Paulo Ferreira, respectively) and existing American
  localizations, version 0.7 is also compatible with non-American English
  dialects for localized punctuation patterns. In your preamble, call Babel
  with the language of your choice: british, canadian, australian, spanish,
  and american should all work equally well (though some newer bibstrings
  remain untranslated in Spanish). Portuguese support is not yet included with
  biblatex.

Changelog for version 0.7 beta:
- added partial support for @suppbook, @suppcollection
- made style definitions independent from sample Biblatex style files
- segregated localizations into external .lbx files
- added comma before name affixes
- added test for comma before "et al.": negative in citations, positive in
  list of Works Cited
- added test for colon before subtitle, returning negative after terminal
  punctuation (such as exclamation point, question mark)
- added "totalnames" entry option for listing all authors and editors in the
  list of Works Cited for a particular entry
- added "uniquetranslator" entry option, used for an @incollection entry with
  its own translator not shared with the rest of the collection
- slightly changed default name dash in Works Cited
- added support for year editions for @inreference works
- improved logic of @video macro
- added support for "eds." before title when editors are plural
- renamed "strict" package option to "footnoterulestrict"
- added draft mode style helper for multiple citations
- added "mladraft" package option for calling style helper outside of draft
  mode
- added localization for "typecompilerandeditor" editortype

Changelog for version 0.6.1:
- IMPORTANT CHANGE: because of difficulties formatting articles without volume
  numbers as newspaper articles, I've had to regress that option sooner than I
  expected. Updated bibtex files by adding the entrysubtype field and setting
  it to "newspaper" or "magazine". Article entries with undefined volume
  fields are now formatted as journal articles without any volume numbers (as
  one might have expected biblatex-mla to have done all along...)
- updated documentation for the above change; added link for installing
  Biblatex from CTAN in installation instructions
- fixed bugs with spacing, problems with spurious punctuation in Reviews, and
  some other minor things
- updated footnote internal macros to use native quotation marks and
  punctuation nesting, thereby fully regressing mkbibquotepunct command
- added "strict" package option after biblatex-chicago-notes-df; feature is
  undocumented for now

Changelog for version 0.6:
- native support for biblatex-, csquote-, and babel-empowered American-style
  punctuation and double quotation marks added in biblatex 0.8 (footnotes not
  yet updated)
- add support for @unpublished, @proceedings, @inproceedings, @periodical
  entrytypes
- add support for published theses
- standardized .bib file keys, strings, fields across entrytypes
- improve minor presentation errors, including misplaced comma before "et al,"
  the size of the name dash in Works Cited (to match that in the Style Manual
  more closely (redefine \mlanamedash to change)), and other things
- simplified and made many internal macros less hack-y and more localizable
- defined many new bibliography strings and redefined existing ones
- commented out issn, isbn, doi, and similar fields as a temporary fix
- allow idem after shorthands in citations
- improved presentation of dates, dropping opening zero
- added support for articles in special issues of journals
- added support for annotated bibliographies using the "annotation" option
- improved support/presentation for subtitles
- usetranslator entry-option now stable, uses native biblatex support
- improved documentation
- add support for nameaddon

Changelog for version 0.5 (final):
- introduction of firstlonghand and nofullnote package options
- changed approach of shorthand citations, defaulting to a "longhand" citation
  for the first citation
- introduction of usetranslator entry option
- fixed more stupid errors
- added support for video and booklet entrytypes
- added hyperlinks for citations with only page numbers
- added better support for useauthor and useeditor entry options
- added location to newspaper articles
- added edition ("version") to newspaper articles (ie, late, national,
  morning, etc.)
- added Spanish localization by Ivan Fernandez

Changelog for version 0.5 (beta):
- introduction of MLA-style footnote citation support
- fixed many more stupid errors (made since the beginning)
- added support for book reviews and reference articles (use "review"
  entrytype and "inreference" entrytype, respectively)
- tidied stylistic problems including erroneous punctuation before URLs
  (pointed out by Stephen Brumbaugh), stray spaces, a few doubled
  punctuations, etc.
- added support for anonymous incollection works (for example, "Beowulf" in an
  English literature anthology shouldn't by default be referenced by the
  editor of that anthology)
- added support for single-author collections (for example, a single poet's
  Collected Poems, with or without a named editor)
- preliminary support for "video" entrytype
- a few other things I'm forgetting

Changelog for version 0.4:
- proper MLA-style crossref support (though Philipp Lehmann's warnings of the
  dangers of crossrefs in Bibtex files still hold: the parent will overwrite
  anything undefined in the child, like Title and Author)
- fixed many stupid errors (made when converting to biblatex 0.7 in version
  0.3)
- introduced logic for idems, ibids, and prenotes (reduces chances of prenotes
  and ibids obscuring the actual author's name)
- changed style name to biblatex-mla to fit in with everything else being
  lowercase
- fixed compatibility with tex4ht (documents made with biblatex-mla can now be
  converted to OpenOffice format easily)
- added support for Newspaper articles (use "article" type, set no volume and
  no issue number)
- added access dates for online articles
- got rid of a couple stray periods lurking in some places.
- defined \fullcite command to provide examples of bibliographic citations (as
  seen in the new samples page)
- added samples page

Changelog for version 0.3:
- updated for compatibility to biblatex 0.7
- incorporated improvements made by Jay Savage regarding URL presentation in
  Works Cited and the handling of edited books lacking authors
- added support for the starred variants of \cite* and \autocite* for citing
  titles when the author is already named in the sentence (e.g., "Joyce says
  many fine things (Ulysses 34)," written as "Joyce says many fine things
  \autocite*[34]{citekey}"). This variation will basically just force skip the
  author's name in a citation. If it's an author with multiple titles in the
  Works Cited, it will list the title and page; otherwise it will list just
  the page.
- added functionality to use first name initials to differentiate among common
  surnames (option uniquename=init made available in biblatex 0.7) in
  citations
- added localizations for "Ed. and trans.," etc. I'm not sure how accurate
  these are yet, but it at least lets us have nicer Works Cited lists. You'll
  see this change when works have a single person responsible for any
  combination of editing, translating, introducing, annotating, or providing
  commentary, forewards, or afterwards. With this change, the person is listed
  only once, with the appropriate words before the name.
- restyled the URL font in the Works Cited to be the same as the rest of the
  documents (as suggested by Jay Savage)
- added support for \cite (same as \autocite) to be more supportive to
  existing programs that assume cite as the command used for references and to
  make conversion easier for newcomers who've already been using \cite
- improved idem handling with boolean triggers
- cleaned up macro names to make them easier to follow



==> Templates/CHANGES <==
Changelog for version 1.9
- changes for compatibility with the latest MLA edition; use "style=mla-new" to change the Works Cited to the new style
- added support for some common biblatex-chicago citation commands (\headlesscite, \textcite, etc.)
- added preliminary support for new entry types (@artwork, @audio, @image, @letter, @music)
- added style intelligence with source mapping:
    * the word "University" in publisher names will automatically shorten to "U"
    * the word "Press" in publisher names will automatically shorten to "P"
    * the phrase "University Press" in publisher names will automatically shorten to "UP"
    * certain words in publisher names--including "Company," "Corporation," "Incorporated", "Limited," and their 
      respective abbreviations--will not be printed
    * if an entry includes a URL pointing to a number of eprint domains--including include JSTOR, Project Muse, Adelaide 
      Online Books, Google Books, EBSCO Academic Search Complete, EBSCO LexisNexis, and the EBSCO MLA Database--
      biblatex-mla will correctly reformat it as an eprint
    * if an entry includes a URL pointing to a doi server, biblatex-mla will correctly reformat it as an doi reference

Changelog for version 1.6
- changes for compatibility with Biblatex 3.3+
- changed behavior of "mancitepar", which now defaults to false
- fixed buggy repetition of series field (hopefully)
- an upcoming version will provide support for more entrytypes and reflect changes made 
  in the 2016 MLA handbook

Changelog for version 1.5:
- changes for compatibility with Biblatex 2.5
- added entrytypes @online, @inbook, @bookinbook
- updated entrytypes @video, @review
- added epprinttype "jstor"
- added package options "noremoteinfo" and "mancitepar" 
- added hyperref linking to "Web" bibstring
- quashed lingering spacing errors, improved bibnamedash, and improved handling of starred
  autocites
- improved documentation, examples

Changelog for version 0.9.5:
- changes for compatibility with Biblatex 1.0
- further support for latest MLA edition (now default); use "showmedium=false" 
  package option to revert
- added Italian localization (from Andrea Marchitelli)
- new entry option "nodate" to trigger display of MLA-style "n.d."
- added support and MLA formatting for eprint sources from Project Muse (using
  "muse" as eprinttype); in the eprint field, include the full URL to the
  article
- preliminary conversion of documentation to Philipp Lehman's ltxdockit, as 
  previous documentation files were lost

Changelog for version 0.9:
- many changes for compatibility with Biblatex v.0.9
- introduced support for style from latest MLA edition (this was a major 
  undertaking)
- new "print", "web", and "generaleditor" bibstrings
- formatting for eprint sources from JSTOR and Google Books, as already 
  included in Biblatex
- support and formatting for eprint sources from eBooks@Adelaide (using 
  "adelaide" as eprinttype); in the eprint field, include the full URL to the
  article
- new package options "showmedium" and "guessmedium" for updated MLA support
- improved support for reprints
- improved support for multivolume entries, including change from using 
  origyear field to using eventdate field, and added support for general 
  editor as "generaleditor" editortype
- converted proceedings to use eventdate field

Changelog for version 0.8.1:
- did nothing but make 0.8 beta final to upgrade CTAN

Changelog for version 0.8 beta:
- added further examples from the MLA Handbook (6th edition). Almost all of
  the non-periodical examples in section 5.6.x (and many of the periodical
  examples in 5.7.x) contained therein can now be successfully re-created
  using biblatex-mla.
- nameaddon and authortype behavior standardized across entrytypes
- added bookauthor support for suppcollection and suppbook
- significantly improved handling of multivolume works
- further improved handling of "et al." There should now be a comma before 
  "et al." only in reversed (last-first) naming schemes. Standard (first-last)
  schemes and last-name only schemes will omit the comma.
- improved support for maintitle
- improved presentation of title in conference proceeding, where title ends in
  an abbreviation dot
- added preliminary support for "generaleditor" editortype in the language
  (lbx) files
- added preliminary support for "volstodate" string in the language (lbx)
  files, theoretically to be used when indicating total volume numbers of
  multi-volume works with open-ranged years
- added title format for reference books
- removed extra leading space before nameaddon brackets
- added support for formatting of open-ranged years (as suggested by 
  Philipp Lehman)
- added support for limiting remote info, using methods similar to
  biblatex-apa
- added totalnames support for translator field
- re-added hyperref support mistakenly disabled in version 0.7
- fixed many citereset problems (while potentially introducing others...)
- many citation macros tidied and future-proofed
- footnote presentation considerably more stable

Changelog for version 0.7 final:
- added examples from the MLA Handbook (6th edition)
- added support for origlocation, origpublisher, origtitle, and origlanguage
  to allow for reprints and translations. Biblatex-mla only uses the
  origlanguage field to trigger the use of \bibstring{transof} in place of
  \bibstring{reprintof} for reprinted articles and will not actually print the
  contents of the origlanguage field.
- re-added support for translators in articles (mistakenly lost in 0.6)
- added localization and bibstrings for "bytypecompilerandeditor" and
  "transof" (in addition to "typecompilerandeditor")
- significantly improved footnote support, bringing it inline with support for
  entries in the bibliography. This work is currently in progress, but non-
  periodical entries should be fully supported.
- in addition to Spanish and Portuguese localizations (contributed by Ivan
  Fernandez and Paulo Ferreira, respectively) and existing American
  localizations, version 0.7 is also compatible with non-American English
  dialects for localized punctuation patterns. In your preamble, call Babel
  with the language of your choice: british, canadian, australian, spanish,
  and american should all work equally well (though some newer bibstrings
  remain untranslated in Spanish). Portuguese support is not yet included with
  biblatex.

Changelog for version 0.7 beta:
- added partial support for @suppbook, @suppcollection
- made style definitions independent from sample Biblatex style files
- segregated localizations into external .lbx files
- added comma before name affixes
- added test for comma before "et al.": negative in citations, positive in
  list of Works Cited
- added test for colon before subtitle, returning negative after terminal
  punctuation (such as exclamation point, question mark)
- added "totalnames" entry option for listing all authors and editors in the
  list of Works Cited for a particular entry
- added "uniquetranslator" entry option, used for an @incollection entry with
  its own translator not shared with the rest of the collection
- slightly changed default name dash in Works Cited
- added support for year editions for @inreference works
- improved logic of @video macro
- added support for "eds." before title when editors are plural
- renamed "strict" package option to "footnoterulestrict"
- added draft mode style helper for multiple citations
- added "mladraft" package option for calling style helper outside of draft
  mode
- added localization for "typecompilerandeditor" editortype

Changelog for version 0.6.1:
- IMPORTANT CHANGE: because of difficulties formatting articles without volume
  numbers as newspaper articles, I've had to regress that option sooner than I
  expected. Updated bibtex files by adding the entrysubtype field and setting
  it to "newspaper" or "magazine". Article entries with undefined volume
  fields are now formatted as journal articles without any volume numbers (as
  one might have expected biblatex-mla to have done all along...)
- updated documentation for the above change; added link for installing
  Biblatex from CTAN in installation instructions
- fixed bugs with spacing, problems with spurious punctuation in Reviews, and
  some other minor things
- updated footnote internal macros to use native quotation marks and
  punctuation nesting, thereby fully regressing mkbibquotepunct command
- added "strict" package option after biblatex-chicago-notes-df; feature is
  undocumented for now

Changelog for version 0.6:
- native support for biblatex-, csquote-, and babel-empowered American-style
  punctuation and double quotation marks added in biblatex 0.8 (footnotes not
  yet updated)
- add support for @unpublished, @proceedings, @inproceedings, @periodical
  entrytypes
- add support for published theses
- standardized .bib file keys, strings, fields across entrytypes
- improve minor presentation errors, including misplaced comma before "et al,"
  the size of the name dash in Works Cited (to match that in the Style Manual
  more closely (redefine \mlanamedash to change)), and other things
- simplified and made many internal macros less hack-y and more localizable
- defined many new bibliography strings and redefined existing ones
- commented out issn, isbn, doi, and similar fields as a temporary fix
- allow idem after shorthands in citations
- improved presentation of dates, dropping opening zero
- added support for articles in special issues of journals
- added support for annotated bibliographies using the "annotation" option
- improved support/presentation for subtitles
- usetranslator entry-option now stable, uses native biblatex support
- improved documentation
- add support for nameaddon

Changelog for version 0.5 (final):
- introduction of firstlonghand and nofullnote package options
- changed approach of shorthand citations, defaulting to a "longhand" citation
  for the first citation
- introduction of usetranslator entry option
- fixed more stupid errors
- added support for video and booklet entrytypes
- added hyperlinks for citations with only page numbers
- added better support for useauthor and useeditor entry options
- added location to newspaper articles
- added edition ("version") to newspaper articles (ie, late, national,
  morning, etc.)
- added Spanish localization by Ivan Fernandez

Changelog for version 0.5 (beta):
- introduction of MLA-style footnote citation support
- fixed many more stupid errors (made since the beginning)
- added support for book reviews and reference articles (use "review"
  entrytype and "inreference" entrytype, respectively)
- tidied stylistic problems including erroneous punctuation before URLs
  (pointed out by Stephen Brumbaugh), stray spaces, a few doubled
  punctuations, etc.
- added support for anonymous incollection works (for example, "Beowulf" in an
  English literature anthology shouldn't by default be referenced by the
  editor of that anthology)
- added support for single-author collections (for example, a single poet's
  Collected Poems, with or without a named editor)
- preliminary support for "video" entrytype
- a few other things I'm forgetting

Changelog for version 0.4:
- proper MLA-style crossref support (though Philipp Lehmann's warnings of the
  dangers of crossrefs in Bibtex files still hold: the parent will overwrite
  anything undefined in the child, like Title and Author)
- fixed many stupid errors (made when converting to biblatex 0.7 in version
  0.3)
- introduced logic for idems, ibids, and prenotes (reduces chances of prenotes
  and ibids obscuring the actual author's name)
- changed style name to biblatex-mla to fit in with everything else being
  lowercase
- fixed compatibility with tex4ht (documents made with biblatex-mla can now be
  converted to OpenOffice format easily)
- added support for Newspaper articles (use "article" type, set no volume and
  no issue number)
- added access dates for online articles
- got rid of a couple stray periods lurking in some places.
- defined \fullcite command to provide examples of bibliographic citations (as
  seen in the new samples page)
- added samples page

Changelog for version 0.3:
- updated for compatibility to biblatex 0.7
- incorporated improvements made by Jay Savage regarding URL presentation in
  Works Cited and the handling of edited books lacking authors
- added support for the starred variants of \cite* and \autocite* for citing
  titles when the author is already named in the sentence (e.g., "Joyce says
  many fine things (Ulysses 34)," written as "Joyce says many fine things
  \autocite*[34]{citekey}"). This variation will basically just force skip the
  author's name in a citation. If it's an author with multiple titles in the
  Works Cited, it will list the title and page; otherwise it will list just
  the page.
- added functionality to use first name initials to differentiate among common
  surnames (option uniquename=init made available in biblatex 0.7) in
  citations
- added localizations for "Ed. and trans.," etc. I'm not sure how accurate
  these are yet, but it at least lets us have nicer Works Cited lists. You'll
  see this change when works have a single person responsible for any
  combination of editing, translating, introducing, annotating, or providing
  commentary, forewards, or afterwards. With this change, the person is listed
  only once, with the appropriate words before the name.
- restyled the URL font in the Works Cited to be the same as the rest of the
  documents (as suggested by Jay Savage)
- added support for \cite (same as \autocite) to be more supportive to
  existing programs that assume cite as the command used for references and to
  make conversion easier for newcomers who've already been using \cite
- improved idem handling with boolean triggers
- cleaned up macro names to make them easier to follow


